Data Poisoning Attacks against Online Learning

We consider data poisoning attacks, a class of adversarial attacks on machine learning where an adversary has the power to alter a small fraction of the training data in order to make the trained classifier satisfy certain objectives. While there has been much prior work on data poisoning, most of it is in the offline setting, and attacks for online learning, where training data arrives in a streaming manner, are not well understood. In this work, we initiate a systematic investigation of data poisoning attacks for online learning. We formalize the problem into two settings, and we propose a general attack strategy, formulated as an optimization problem, that applies to both with some modifications. We propose three solution strategies, and perform extensive experimental evaluation. Finally, we discuss the implications of our findings for building successful defenses.

==> attacks.tex <==
\section{Attack Methods}
\label{sec:attacks}

In the setting described above, finding the attacker's optimal strategy reduces to solving a certain attack optimization problem. We begin by describing this problem.

In the sequel, given a data stream $S$, we use the notation $S_t$ to denote the $t$-th labeled example in the stream. Additionally, the difference between two data streams $S$ and $S'$, denoted by $S \setminus S'$, is defined as the set $\{ S_t | S_t \neq S'_t \}$; its cardinality $| S \setminus S'|$ is the number of of time steps $t$ for which $S_t \neq S'_t$. 

\subsection{Attacker's Optimization Problem} 

Under this notation, the attacker's optimal strategy under an input data stream $\Strain$ in the semi-online case can be described as the solution to the following optimization problem.

%\begin{equation}
\begin{align}
& \max_{S \in \calF^T} \bbE_{(x, y) \sim D} \mathds{1} (\sgn(w_T^{\top} x) \neq y) \\
& \mbox{subject to:} && | S \setminus \Strain | \leq K, \label{eqn:L0constraint} \\
&&& w_t = w_0 - \sum_{\tau=0}^{t-1} \eta_{\tau} ( \grad \ell (w_{\tau}, S_{\tau}) + \grad \Omega(w_{\tau})), 1 \leq t \leq T \label{eqn:OGDconstraint}
\end{align}
%\end{equation}

Here, \eqref{eqn:L0constraint} ensures that at most $K$ examples in the input data stream are changed, and \eqref{eqn:OGDconstraint} ensures that $w_t$ is the OGD iterate at time $t$. In the fully online case, the objective changes to $\sum_{t=1}^{T} \bbE_{(x, y) \sim D}\mathds{1} (\sgn(w_t^{\top} x) \neq y)$.

%\yz{We start with stating the optimization problem which the attacker needs to solve. Let $\Sorigin$ be the clean training data stream, $S = \{(x_0, y_0), \cdots, (x_{T-1}, y_{T-1})\}$ be the length $T$ training data stream supplied by the attacker to the online learner, and $w_{S,t}$ be the model parameter of classifier at time $t$.
%For the online logistic regression classifier described in Section~\ref{sec:setting}, the optimization problem becomes
%\begin{equation}
%\begin{aligned}
%&\max_S & & \bbE_{(x,y) \sim \mathcal{D}} \mathds{1}[sgn (w_{S,T}^Tx)\neq y] \\
%&\mbox{subject to}  & & |S\backslash S_{orig}| \leq K, \\
%& & & x_i \in \calF\ \forall x_i \in S, \\
%& & & w_{S,T} = w_0 - \sum_{i=0}^{T-1}\grad l_i(w_i, x_i, y_i).
%\end{aligned}
%\end{equation}
%for the semi-online setting, and
%\begin{equation}
%\begin{aligned}
%&\max_S & & \sum_{t=1}^T\bbE_{(x,y) \sim \mathcal{D}} \mathds{1}[sgn (w_{S,T}^Tx)\neq y] \\
%&\mbox{subject to}  & & |S\backslash S_{orig}| \leq K, \\
%& & & x_i \in \calF\ \forall x_i \in S, \\
%& & & w_{S,t} = w_0 - \sum_{i=0}^{t-1}\grad l_i(w_i, x_i, y_i).
%\end{aligned}
%\end{equation} 
%for the fully-online setting.}




% This, along with the online nature of the problem makes gradient computation more challenging. Perturbing a point $x_t$ now influences all later $w_{\tau}$s, and the KKT conditions, that were exploited by prior work for easy gradient computation, no longer hold at each $w_t$. 

%The second challenge is that because data order matters, the search space for $S$ now includes data points $(x_t, y_t)$ as well as their positions in the stream, which vastly increases the number of search possibilities. 

%presents two additional challenges

%While there have been successful data-poisoning attacks against offline learning algorithms \cite{biggio2012poisoning,steinhardt2017certified}, two additional challenges need to be addressed in order to find an effective attack method against an online algorithm. The first challenge is to quantify the impact of perturbing points in the data stream to the attacker's objective functions. This task can be significantly harder than in the offline case because perturbation at an early points $x_i$ will affect all model parameters $w_{S, j}$ and objective functions for $j > i$. Each $w_{S, j}$ is also a complex nonlinear function of preceding points $x_i$ where $i < j$. Moreover, because the model parameters at each time step are not guaranteed to be the loss minimizer of the entire training stream, the influence function trick using KKT condition at stationary points does not apply. The second challenge is to find the right training points and locations to attack, given that the attacker can only pick a subset of points to perturb. It is computationally prohibitive to try all combinations of attack positions, and the set of legitimate data stream $S$ is also non-convex.

%In this section, we introduce a principled approach to search the optimal data stream that maximizes the attacker's reward function, and propose two attack algorithms that maximize the semi-online and fully-online classification error for an online logistic regression classifier trained using online gradient descent. \yz{The term `principled approach' may sound like a too big promise...}

\subsection{Attack Algorithm}

\paragraph{Challenges.} Observe that this optimization problem has some similarities to the corresponding offline problem derived by~\cite{meizhu2015}. However, there are two important differences that leads to a difference in solution approaches. 

The first is that unlike the offline case where the estimated $\hat{w}$ is the minimizer of an empirical risk, here $w_t$ is a more complex function of the data stream $S$. This has two consequences that make gradient computation more challenging -- first, changing $x_t$ now influences all later $w_{\tau}$ for $\tau > t$; second, the KKT conditions that were exploited by prior work for easy computation no longer hold. 

The second difference from the offline case is that data order now matters, which implies that modifying training points at certain positions in the stream may yield high benefits. This property could be potentially exploited by a successful attack to reduce the search space.

% has the potential to be exploited by a successful attack to 
%Thus, a good attack needs to 
%However, it still  these specific positions are still hard to find. 
%This should be incorporated into any successful solution strategy. 

\paragraph{Our Approach.} We next provide a solution approach that involves three steps, corresponding to our three key ideas.

Our first key idea is to simplify the optimization problem by smoothing the objective function followed by a novel tool -- {\em{label inversion}}; this encourages the attacker to modify the data stream to fit a dataset whose labels are inverted with respect to the original data distribution and removes some local maxima in the process. Second, we show how to compute the gradient of the objective function with respect to points in the data stream by use of the chain rule. Our third key idea is to narrow the search space by confining our search to specific positions in the data stream. We next describe each of these steps. 

%\kc{This introductory paragraph may need to rewritten after we fix the three steps.}

%\kc{We need to address (a) the label yts (b) the feasible set $\calF$}

%consists of the following three components:
%\begin{enumerate}
%\item
%smoothing the objective function if necessary,
%\item
%computing the gradient of the objective function with respect to points in the data stream, and
%\item
%finding the right positions/points in the data stream to attack.
%\end{enumerate}

%In the rest of the section, we propose a effective differentiable surrogate of the 0-1 loss function, a detailed method of computing the exact gradient and three ways of narrowing the search space of the attack positions, which lead to three different attack algorithms, namely the incremental, the interval and the teach-reinforce attack.

%\subsubsection{Smoothing the Attacker's Objective Function}

\subsubsection{Key Idea 1: Simplify Optimization Problem by Label Inversion}

%\kc{what does not come across in this section is that the label inversion trick is novel}
\kc{need to emphasize label inversion}

We begin by observing that the objective function~\eqref{eqn:objective} is not suited for gradient ascent. First, being a $0/1$ loss, it is non-differentiable, and second, it involves an expectation over $\calD$ which we cannot compute as $\calD$ is generally unknown.  This is readily addressed by standard tools -- we use a convex surrogate, the logistic loss, instead of the $0/1$ loss, and evaluating the expectation over a separate validation data set $\Svalid$ \cite{biggio2012poisoning}. \kc{citation for this?}

%For the semi-online case, the modified objective is now:

%\begin{equation} \label{eqn:modifiedobj1}
%\max_{S \in \calF^{T}} \sum_{(x,y)\in \Svalid} \log(1+\exp(-yw_T^{\top} x))
%\end{equation}

%An analogous objective applies to the fully online case. 

However, observe that the new surrogate objective function has a local maximum at the constant classifier. To address this, we propose a novel {\em{label inversion}} procedure. Instead of maximizing logistic loss on the validation set, we construct an inverted validation set $\Sinv$, which contains, for each $(x, y)$ in the validation set, an example $(x, -y)$. We then maximize the negative of the logistic loss on this inverted validation set.

Formally, for an example $(x, y)$ and a weight vector $w$, let $L(w, (x, y))$ denote the negative logistic loss $L(w, (x, y)) = - \log(1 + \exp(-y w^{\top} x))$.  For the semi-online case, the objective~\eqref{eqn:objective} reduces to $\max_{S \in \calF^{T}} L(S) = \max_{S \in \calF^{T}} \sum_{(x,y)\in \Sinv} L(w_T, (x, y))$. 

%\begin{equation} \label{eqn:modifiedobj2}
%\end{equation}

Intuitively, this encourages the attacker to modify the data stream to fit a dataset whose labels are inverted with respect to the original data distribution. Again, an analogous objective can be derived for the fully online case. 
 
%preprocessing, where we instead minimize the logistic loss on a {\em{modified}} validation set whose features remain the same, but labels have opposite signs. Intuitively, the attacker attacker is forcing the online algorithm to fit a dataset whose label is the opposite to the underlying distribution. 


%Suppose we have a logistic regression classifier with weight $w$ that always predicts $+1$, and assume the true label of data drawn from $\mathcal{D}$ is balanced between $-1$ and $+1$. The classifier will be wrong about half of the time. In appendix~\ref{proof:localmaxima}, we show that by making more extreme prediction, i.e. increasing the prediction score $w^Tx$ of both positive and negative instances, we will obtain an increasing logistic loss over the validation set. We also observe that empirically the attacking algorithm tends to find the data stream $S$ that leads to such an extreme constant classifier even when it is allowed to arbitrarily perturb all points in the original data stream $S_{orig}$, which apparently is not the optimal attack. \yz{TODO: write a proof to show this point.} 


%Our first observation is that the objective function 
%The objective function $f_t(S) = \bbE_{(x,y)\sim\mathcal{D}} \mathds{1}[A_{S,t}(x) \neq y]$ for the attacker is in general not differentiable. A standard surrogate objective is the logistic loss over a validation set drawn from $\mathcal{D}$. Specifically, let $S_{valid}$ be the validation set, and $w_{S,t}$ be the model parameter of the logistic regression classifier $A_{S,t}$ at time $t$. The attacker's objective at time step $t$ for a training data stream $S$, denoted by $L_t(S)$, is
%\begin{equation}
%L_t(S) = \sum_{(x,y)\in \Svalid} \log(1+\exp(-yw_{S,t}^Tx)).
%\end{equation}
%The attacker wants to maximize 
%\begin{equation}
%L(S) = L_T(S) = \sum_{(x,y)\in \Svalid}\log(1+\exp(-yw_{S,T}^Tx))
%\end{equation}
%for the semi-online setting, and
%\begin{equation}
%    L(S) = \sum_{t=1}^T L_t(S) = \sum_{(x,y)\in \Svalid}\sum_{t=1}^T\log(1+\exp(-yw_{S,t}^Tx))
%\end{equation}
%for the fully-online setting.

%Intuitively, the performance on the validation set is a good gauge of that on the data distribution, and larger loss often corresponds to an increasing number of classification errors. However, this standard surrogate can be misleading in the online logistic regression case because it often has a local maximum at a constant classifier. Suppose we have a logistic regression classifier with weight $w$ that always predicts $+1$, and assume the true label of data drawn from $\mathcal{D}$ is balanced between $-1$ and $+1$. The classifier will be wrong about half of the time. In appendix~\ref{proof:localmaxima}, we show that by making more extreme prediction, i.e. increasing the prediction score $w^Tx$ of both positive and negative instances, we will obtain an increasing logistic loss over the validation set. We also observe that empirically the attacking algorithm tends to find the data stream $S$ that leads to such an extreme constant classifier even when it is allowed to arbitrarily perturb all points in the original data stream $S_{orig}$, which apparently is not the optimal attack. \yz{TODO: write a proof to show this point.} 

%We overcome this problem by using the logistic loss on a modified validation set whose labels are flipped from the original as the surrogate objective, and then trying to minimize such loss function. Intuitively, the attacker is forcing the online algorithm to fit a dataset whose label is the opposite to the underlying distribution. Let $\Svalid$ be the original validation set drawn from $\mathcal{D}$. For consistency purpose, we use the negative logistic loss on the label-flipped validation set as the attacker's objective so that the attacker still maximizes its objective. Formally, the attacker's objective $L_t(S)$ at time $t$ now becomes 
%\begin{equation}
%L_t(S) = \sum_{(x,y)\in \Svalid} -\log(1+\exp(yw_{S,T}^Tx))
%\end{equation}
%The attacker wants to maximize 
%\begin{equation}
%    L(S) = L_T(S) = \sum_{(x,y)\in \Svalid} -\log(1+\exp(yw_{S,T}^Tx))
%\end{equation}
%for the semi-online setting, and
%\begin{equation}
%    L(S) = \sum_{t=1}^T L_t(S) = \sum_{(x,y)\in \Svalid}\sum_{t=1}^T -\log(1+\exp(yw_{S,t}^Tx))
%\end{equation}
%for the fully-online setting. The loss due to a constant classifier is no longer a local extremum for this surrogate objective.

\subsubsection{Key Idea 2: Compute Gradients via Chain Rule}

The next challenge is how to compute the gradient of the objective function with respect to a training point $(x_t, y_t)$ at position $t$. Unlike the offline case, this is more challenging as the KKT conditions can no longer be used, and the gradient depends on position $t$. Our second observation is that this can still be achieved by judicious use of the chain rule.

We first observe that in the optimization problem~\eqref{eqn:objective}, replacing a training point $(x_t, y_t)$ with $(-x_t, -y_t)$ leads to exactly the same result; this is due to symmetry of the feasible set as well as the OGD algorithm. We therefore choose to keep the label $y_t$'s fixed in the training set, and only optimize over the feature vector $x_t$s. 

%logistic regression classifiers learned using OGD, replacing a point $(x_i, y_i)$ with $(-x_i, -y_i)$ will give the exactly the same update and results. In other words, if the optimal solution contains $(x_i,y_i)$, replacing $(x_i, y_i)$ with $(-x_i, -y_i)$ will result in the same objective function. Since our feasible set is symmetrical around the origin, $(x_i, y_i)$ and $(-x_i, -y_i)$ will both be in the feasible set $\calF$. Therefore we can just optimize over all $x_i$ in the data stream $S$.


Let $(x, y)$ be an example in the inverted validation set $\Sinv$. Using Chain Rule, the gradient of the loss $L(w_t, (x, y))$ with respect to the training point $(x_i, y_i)$ can be written as:

\kc{Yizhen can you fix the notation -- $L(w, (x, y))$?}

\begin{equation}
    \frac{\pd L(w_t,x,y)}{\pd x_i} = \left\{
    \begin{array}{ll}
         0 & \mbox{if $i\geq t$}\\
         \frac{\pd L(w_t, x, y)}{\pd w_{t}}\frac{\pd w_{t}}{\pd x_i}&  \mbox{if $i=t-1$}\\
         \frac{\pd L(w_t, x, y)}{\pd w_{t}}\frac{w_{t}}{w_{t-1}}\cdots \frac{w_{i+2}}{w_{i+1}}
    %\left(\prod_{s=i+1}^{t-1}\frac{\pd w_{s+1}}{\pd w_{s}}\right) 
    \frac{\pd w_{i+1}}{\pd x_i} & \mbox{if $i<t-1$}.
    \end{array}\right\}
\end{equation}

%\kc{Isn't $\pd L (w_t)/\pd x_t = 0$? I thought that only $w_{t+1}$ depends on $x_t$, no?}
Each of the terms $\frac{\pd L(w_t, x, y)}{\pd w_t}$, $\frac{\pd w_{s+1}}{\pd w_{s}}$ and $\frac{\pd w_{i+1}}{\pd x_i}$ may be recursively calculated directly; a detailed derivation is given in the Appendix. The full gradient of the objective $L(S)$ may now be computed by summing over the gradients of $L(w, (x, y))$ for $(x, y)$ in $\Sinv$. \kc{Yizhen can you prep this part in the Appendix?}

%\kc{This is not written quite right...}

%\kc{what about gradient with respect to $y_i$ here?}

% let the corresponding 
%One way to quantify the impact of a perturbation to the objective and also one vital step for any gradient ascent method is to find the gradient of the objective w.r.t. to the input variables, in this case the training points $(x_0, y_0), \cdots, (x_{T-1}, y_{T-1})$. Let $x_i$ denote the input instance at the $i$-th time step and $y_i$ the label of it. If the feasible set for each $x_i$ in the data stream is $[-1, 1]^d$, then it suffices to only perturb $x_i$ because if the optimal attack contains $(x_i, y_i)$ at the $i$-th step, replacing the point with $(-x_i, -y_i)$ will result in the same updates for model parameters and therefore the same objective function value. We show that the gradient $\pd L_t(S) / \pd x_i$ can be computed analytically for an online logistic regression classifier. 

%Let $w_t$ be the model parameter and $L(w_t, x, y) = -\log(1+\exp(yw_t^Tx))$ be the attacker's objective function on a point $(x,y)$ at time step $t$, then
%\begin{equation} 
%\begin{split}
%    \frac{\pd L_t(S)}{\pd x_i} =&\ \sum_{(x,y) \in \Svalid} \frac{\pd L(w_t, x, y)}{\pd x_i}.
%\end{split}
%\end{equation}
%By chain rule,
%\begin{equation}
%    \frac{\pd L(w_t,x,y)}{\pd x_i} = \left\{
%    \begin{array}{ll}
%         0 & \mbox{if $i>t$}\\
%         \frac{\pd L(w_t, x, y)}{\pd x_i} & \mbox{if $i=t$}\\
%         \frac{\pd L(w_t, x, y)}{\pd w_t}\frac{\pd w_t}{\pd x_i}&  \mbox{if $i=t-1$}\\
%         \frac{\pd L(w_t, x, y)}{\pd w_t}
%    \left(\prod_{s=i+1}^{t-1}\frac{\pd w_{s+1}}{\pd w_{s}}\right) \frac{\pd w_{i+1}}{\pd x_i} & \mbox{if $i<t-1$}.
%    \end{array}\right.
%\end{equation}
%where 
%\begin{equation}
%    \frac{\pd L(w_t, x, y)}{\pd w_t}
%    = -\frac{yx}{1+\exp(-yw_t^Tx)} + 2\lambda w_t,
%\end{equation}
%\begin{equation}
%\begin{split}
%    \frac{\pd w_{s+1}}{\pd w_s} =\ (1-2\lambda\eta_s)\identity - \eta_s\left(\frac{\exp(y_sw_s^Tx_s)}{[1+\exp(y_sw_s^Tx_s)]^2}\right)x_sx_s^T,
%\end{split}
%\end{equation}
%and 
%\begin{equation}
%\begin{split}
%    \frac{\pd w_{i+1}}{\pd x_i} =\  -\eta_t\left(
%    \frac{-y_i\identity}{1+\exp(y_iw_i^Tx_i)}
%    + \frac{\exp(y_iw_i^Tx_i)x_iw_i^T}{[1+\exp(y_iw_i^Tx_i)]^2}
%    \right).
%\end{split}
%\end{equation}

%Finally, by linearity of gradients of continuous functions, we obtain
%\begin{equation}
%\frac{\pd L(S)}{\pd x_i} = \frac{\pd L_T(S)}{\pd x_i}
%\end{equation}
%for the semi-online setting, and 
%\begin{equation}
%\frac{\pd L(S)}{\pd x_i} = \sum_{t=1}^T\frac{\pd L_t(S)}{\pd x_i}
%\end{equation}
%for the fully-online setting.

\subsubsection{Key Idea 3: Strategic Search over Positions in the Stream}

So far, we have calculated the impact of modifying a single point $(x_t, y_t)$ on the objective function; a remaining question is which data points in the input stream to modify. Recall that in a data stream of length $T$, there are potentially $\binom{T}{K}$ subsequences of $K$ inputs to modify, and a brute force search over all of them is prohibitively expensive. We present below three algorithms for strategically searching over positions in the stream for attack purposes -- the Incremental Attack, the Interval Attack and the Teach-and-Reinforce Attack. 

A first idea is to consider a {\em{greedy approach}}, which iteratively alters the training point in the sequence that has the highest gradient magnitude. While this has been considered by prior work for offline settings, we next derive how to do this in an online setting. This results in what we call the {\em{Incremental Attack}}.

\paragraph{Incremental Attack.} This attack employs an iterative steepest coordinate descent approach. In each iteration, we calculate the gradient of the modified objective~\eqref{eqn:modifiedobj} with respect to each single training point, and pick the $(x_{t}, y_{t})$ with the largest gradient magnitude. This example is then updated as: 
\[ x_{t} \leftarrow x_{t} + \epsilon \proj_{\calF}(\pd L(S) / \pd x_{t}), \]
where $\epsilon$ is a step size parameter, $L(S)$ is the objective function, and $\proj$ is the projection operator. The process continues until either $K$ distinct points are modified or convergence. The full algorithm is described in Algorithm~\ref{algo:incremental} in the Appendix.

% $\pd L(S) / \pd x_i$ for all $(x_i, y_i) \in S$. It then picks a single training points $(x_i, y_i)$ where the gradient of attacker's objective has the largest norm, i.e.
%\begin{equation}
%\arg\max_{x_i \in S} ||\frac{\pd L(S)}{\pd x_i}||_2,
%\end{equation} 
%and updates $x_i$ to $x_i + \eta \pd L(S) / \pd x_i$, where $\eta$ is the step size. The attack stops when either $K$ distinct points are modified or the objective function converges. The full algorithm description is in Algorithm~\ref{algo:incremental}.

%Observe however that the greedy approach has two limitations. The first is that it does not take into account the online nature of the problem, and is hence involves a large number of iterations, which may be expensive to run in the online setting. The second is that it is known to be prone to local minima. \kc{cite percy}

Observe however that the greedy approach has two limitations. The first is that since it does not narrow the search space using the online nature of the problem, it involves a large number of iterations and is computationally expensive. The second is that it is known to be prone to local minima as observed by prior work in the offline setting. \cite{steinhardt2017certified}


\paragraph{Interval Attack.} To address these limitations, we next propose a novel strategy that is tailored to the online setting, called the {\em{Interval Attack}}. The idea here is to find the  best {\em{consecutive sequence}} $(x_t, y_t), \ldots, (x_{t + K -1}, y_{t+K-1})$ modifying which decreases the objective function the most. Since this reduces the search space, the attack has a lower running time.

%More specifically, for each $0 \leq t \leq T - K$, the algorithm finds the concatenated gradient of the objective $L(S)$ $[\pd L(S)/\pd x_{t}, \cdots, \pd L(S)/\pd x_{t+K-1}]$, and select the $t$ for which this gradient has the highest magnitude. Once $t$ is chosen, successive iterations are carried out for the same $t$ until convergence. Each iteration carries out the update:
%\[ [x_t, \cdots, x_{t+K-1}] \leftarrow [x_t, \cdots, x_{t+K-1}] + \epsilon \proj_{\calF^K}([\pd L(S)/\pd x_{t}, \cdots, \pd L(S)/\pd x_{t+K-1}]) \]
%where $\epsilon$ is again a step-size parameter, $L(S)$ is the objective. 

More specifically, the search process is as follows. For each $t \in \{ 0, \ldots, T - K - 1\}$, the algorithm computes the concatenated gradient $[\pd L(S)/\pd x_{t}, \cdots, \pd L(S)/\pd x_{t+K-1}]$ and carries out the following update until convergence or until a maximum number of iterations is reached:
\[ [x_t, \cdots, x_{t+K-1}] \leftarrow [x_t, \cdots, x_{t+K-1}] + \epsilon \proj_{\calF^K}([\pd L(S)/\pd x_{t}, \cdots, \pd L(S)/\pd x_{t+K-1}]), \]
where $\epsilon$ is again a step-size parameter. The value of $t$ for which the final $[x_t, \ldots, x_{t + K -1}]$ gives the best objective~\eqref{eqn:objective} is then selected. 


%The final value of $[x_t, \ldots, x_{t+K-1}]$ obtained is then used to determine the maximum bene

%Here $\epsilon$ is again a step-size parameter. 

%In the interval attack, the attacker modifies all points within a consecutive time window, whose length is the attacker's budget $K$. The search space is then reduced to the start time $t$ of the windows. Once an interval is chosen, the attack iterates over the same interval. In each iteration, the algorithm finds the concatenated gradient $[\pd L(S)/\pd x_{t}, \cdots, \pd L(S)/\pd x_{t+K-1}]$, and updates $[x_t, \cdots, x_{t+K-1}]$ to $[x_t, \cdots, x_{t+K-1}] + \eta[\pd L(S)/\pd x_{t}, \cdots, \pd L(S)/\pd x_{t+K-1}]$. It stops when either the objective function converges or the maximum number of iteration is reached. After searching over all candidate intervals, the attacker modifies the interval that gives the best attack outcome on the validation set. The full algorithm description is at Algorithm~\ref{algo:interval}. 


\paragraph{Teach-and-Reinforce Attack.} Even though the Interval attack is faster than the Incremental, it has the highest impact on the performance of the classifiers $w_{t'}$ for $t'$ close to $t$. In particular, it is suboptimal in the fully online case, where the objective is the sum of the losses of all $w_t$. This motivates our third attack strategy -- the {\em{Teach-and-Reinforce Attack}}, which seeks to first {\em{teach}} a new classifier by modifying a set of initial examples, and then {\em{reinforce}} the teaching by modifying examples along the rest of the data stream.

We split $K$, the number of examples to be modified, into two parts $\alpha K$ and $(1 - \alpha)K$. We then modify the first $\alpha K$ points in the stream, followed by every $s$-th remaining point, where $s = \lceil \frac{T-\alpha K}{(1-\alpha) K}\rceil$. As in previous attacks, once the attack positions are determined, the algorithm iteratively finds the best modification through gradient ascent followed by projection to the feasible set. The full algorithm is described in Algorithm~\ref{algo:teachreinforce}. Finally, the optimal value of $\alpha$ is determined through a grid search. Observe that $\alpha=0$ corresponds to modifying points over an uniform grid of positions in the stream, and hence the performance of Teach-and-Reinforce is at least as good as this case. 
 


% Intuitively, the attacker `teaches' the online learner a wrong classifier by modifying the first $\alpha K$ points, and constantly `reinforces' the wrong concept taught using its remaining budget. The search space is reduced to the hyper-parameter $\alpha \in [0, 1]$, which can be found by grid search. Let $t = \alpha K$ be the number of modifications for teaching and $s = \lfloor \frac{T-\alpha K}{(1-\alpha) K}\rfloor$ be the distance between two reinforcement points. The attacker iteratively finds the best modification on $[x_0, \cdots, x_{t-1}, x_{t-1+s}, \cdots, x_{t-1+(K-t)s}]$. In each iteration, the attacker finds the gradient $\grad L(S) = [\pd L(S) / \pd x_0, \cdots, \pd L(S) / \pd x_{t-1}, \pd L(S)/ \pd x_{t-1+s}, \cdots, \pd L(S)/ \pd x_{t-1+(K-t)s}]$, and makes the following update  
%$$[x_0, \cdots, x_{t-1}, x_{t-1+s}, \cdots, x_{t-1+(K-t)s}] \leftarrow [x_0, \cdots, x_{t-1}, x_{t+s}, \cdots, x_{t-1+(K-t)s}] + \eta \grad L(S).$$ 
%The attack for a specific $\alpha$ stops when either the objective converges or the maximum number of iteration is reached. The attacker picks the $\alpha$ and its corresponding modification that gives the best attack outcome on the validation set. The full algorithm description is at Algorithm~\ref{algo:teachreinforce}.


